SpectreRewind: Leaking Secrets to Past Instructions

Transient execution attacks utilize micro-architectural covert channels to leak secrets that should not have been accessible during logical program execution. Commonly used micro-architectural covert channels are those that leave lasting footprints in the microarchitectural state, for example, a cache state change, from which the secret is recovered after the transient execution is completed. In this paper, we present SpectreRewind, a new approach to create contention based covert channels for transient execution attacks. In our approach, a covert channel is established by issuing the necessary instructions logically before the transiently executed victim code. Unlike prior contention based covert channels, which require simultaneous multi-threading (SMT), SpectreRewind supports single hardware thread based covert channels, making it viable on systems where attacker cannot utilize SMT. We show that contention on the floating point division unit on commodity processors can be used to create a high-performance (~100 KB/s), low-noise covert channel for transient execution attacks instead of commonly used flush+reload based cache covert channels. We implement a Meltdown attack utilizing the proposed covert channel showing competitive performance compared to the stateof-the-art cache based covert channel implementation. We also show that the covert channel works in the JavaScript engine of a Chrome browser.

==> MDS_POC.tex <==
\section{SpectreRewindMDS POC}\label{sec:MDS_POC}

==> oldfiles/ConSpectre.tex <==
\section{ConSpectre}\label{sec:spectreguard}

\begin{figure}[htp]
  \includegraphics[width=0.5\textwidth]{figs/ROB_in_order.png}
  \caption{Simplified representation of speculative execution attack.}
  \label{fig:ROB_in_order}
\end{figure}

\subsection{Attack Model}
We begin by considering the representation of a speculative execution attack shown in Figure~\ref{fig:ROB_in_order}. In this figure, we place all micro-operations that the processor's front-end has passed into the execution engine in the order that they arrived, we also number them in the order that they arrived. We group together the micro-operations into three distinct sections. Section A consists of micro-operations that arrived before the trigger that will start the malicious mis-speculation. While this section may contain micro-operations that were mis-speculated and squashed, we only focus on the micro-operations that are retired, and whose state becomes visible to the architecture. Section C has the same properties as Section A, but the micro-operations in this section arrived after the micro-operations of the Section B.

Section B contains all of the micro-operations that were executed due to the malicious mis-speculation caused by the attacker. All of the micro-operations in this section are squashed before they reach the head of the ROB and thus, they cannot directly modify the architectural state of the system. Because these micro-operations were not supposed to be executed, it follows that they operate in a way that was not intended by the programmer. This allows these micro-operations to access secret data that – under normal program execution – should have not been accessible. Because the micro-operations of Section B know the value of the secret, but cannot convey that value through the architectural state to micro-operations in Sections A and C, it will instead be the goal of these micro-operations to transmit the value of the secret into a microarchitectural side channel – in Figure~\ref{fig:ROB_in_order} shown as the cache state – that can then be received by micro-operations in Sections A and C, by modifying the execution time of those micro-operations. As most architectures provide timers that can accurately perceive these timing changes, this bridges the gap and allows the mis-speculated instructions to communicate secret information to the architecture.

\subsection{Attack Direction}
\begin{figure}[htp]
  \includegraphics[width=0.5\textwidth]{figs/ROB_out_order.png}
  \caption{Simplified representation of out-of-order speculative execution attack. Here, an older instruction is able to modify the execution of a younger instruction. }
  \label{fig:ROB_out_order}
\end{figure}
While Figure~\ref{fig:ROB_in_order} can help to visualize speculative execution attacks, it may give the false impression that micro-operations from Section B cannot transmit secret data by modifying the execution times of micro-operations from Section A. In reality, modern machines operate using out-of-order execution, and micro-operations from Section B can be executed before micro-operations from Section A. We redraw our diagram to emphasise this property as shown in Figure~\ref{fig:ROB_out_order}. In this Figure, micro-operations appearing above other micro-operations are executed earlier, and micro-operations that are on the same level - e.g. uop2, uop4, and uop6 - are executing at the same time. It should now be easy to see the micro-operations from section B, while in the reorder buffer much later than micro-operations from section A, can be executed much earlier than those same instructions, allowing them to modify the timing of those micro-operations. This leads us to the concept of attack direction. We will say that an attack is forward facing if the maliciously mis-speculated instructions from section B are attempting to transmit secret data to instructions located within sections C, and we will say that the attack is backwards facing if they are trying to transmit to instructions located in section A. It is important to note that the micro-operations within the sections may also execute out-of-order - e.g. uop2 executing before uop1 - because of this, and to keep the diagrams simple, from now on, we only list the most important instructions / micro-operations, and do not list the order that they were inserted into the execution engine.

\subsection{Attack Timing}

\begin{figure}
    \centering
    \begin{subfigure}[a]{0.3\textwidth}
        \includegraphics[width=\textwidth]{figs/timing_exclusive.png}
        \caption{Exclusive Timing}
        \label{fig:time_exclusive}
    \end{subfigure}
    ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
      %(or a blank line to force the subfigure onto a new line)
      
    \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=\textwidth]{figs/timing_inclusive.png}
        \caption{Inclusive Timing}
        \label{fig:time_inclusive}
    \end{subfigure}
    ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
    %(or a blank line to force the subfigure onto a new line)
    
    \begin{subfigure}[c]{0.3\textwidth}
        \includegraphics[width=\textwidth]{figs/timing_incorrect.png}
        \caption{Not Allowed Timing}
        \label{fig:time_incorrect}
    \end{subfigure}
    \caption{Allowed timing strategies.The attacker is limited to a timer that creates a boundary that speculation cannot cross. This leaves two strategies for the timing phase of the attack. }\label{fig:timing}
\end{figure}

All speculative execution attacks require the use of timers to read from the microarchitectural side channel. While high accuracy timers can be created that do not disrupt the malicious mis-speculation, and thus can take timing samples concurrently while micro-operations from Section B are executing, we will assume that the attacker does not have this luxury. We assume that when the attacker takes a time sample, that all micro-operations from Section B have either not begun execution, or have all completed execution. We find that this restriction on the attacker's abilities leads to two possible timing strategies. The first strategy, shown in Figure~\ref{fig:time_exclusive}, will be to start and stop the timer both within Section A or in Section C. As starting and stopping the timer in Section A will time a set of micro-operations that must be executed before the transient section, this strategy will be useless. On the other hand, timing that begins and ends within Section C will occur completely after Section B has executed, which will allow for side channel transmission. As the maliciously mis-speculated micro-operations will fall completely outside of the timing window, we will label attacks that utilize this method as exclusive attacks. The second strategy, shown in Figure~\ref{fig:time_inclusive}, is to begin the timer in Section A of the code, and stop the timer in Section C. This will place the all maliciously mis-speculated micro-operations within the timing window. We will label attacks that utilize this timing method as Inclusive attacks.

\subsection{Stateful vs Concurrent side channels}
Because mis-speculated micro-operations cannot effect the architectural state of the machine, every speculative execution attack requires a microarchitectural side channel. All such side channels work by causing contention on the shared resources of the system's microarchitecture, but they can be classified into two categories. The first we will call stateful side channels, as the side effects caused by accessing the shared resource can modify the execution times of subsequent micro-operations that attempt to access the resource, even after the micro-operations that performed the initial access have been retired. The second type of side channel we will call concurrent, as they depend on the transmitting micro-operations to cause contention by accessing the shared resource concurrently with the receiving micro-operations. We include, in this category, all resource requests that are made by a micro-operation that would no longer cause resource contention once the micro-operation has retired. This means that even if the micro-operation has been squashed - e.g. a load instruction that is squashed after sending the load request into the memory system - it may still cause concurrent contention on resources that it has already made requests to.

\subsection{Example 1: Forward Facing Stateful Exclusive}

\begin{figure}[h]
\begin{verbatim}
       if (x < A.length) {  // mis-speculated here
           secret = A[x];   // access secret
           secret *= 256    // scale secret
           tmp = P[secret]  // secret value to cache
       }
\end{verbatim}
\caption{A Spectre gadget. Adopted from~\cite{kocher2018spectre}}
\label{fig:spectregadget}
\end{figure}

\begin{figure}[htp]
  \includegraphics[width=0.5\textwidth]{figs/spectre_v1.png}
  \caption{The original Spectre variant 1 attack in timing diagram form. We classify such an attack as a Forward Facing Stateful Exclusive attack. }
  \label{fig:spectre_v1}
\end{figure}

Many of the proof of concept attacks presented in previous works fall into the category of forward facing stateful exclusive attacks. We can see an example of this utilizing the original Spectre variant 1 attack code, shown in Figure~\ref{fig:spectregadget}. We show the timing diagram of the attack in Figure~\ref{fig:spectre_v1}, where for clarity, we have replaced micro-operations with the C code that will become those operations. The solid arrows within the section blocks represent the statements that are taking time to fully execute. In this example, the attacker has mis-trained statement 1, such that even though x is out-of-bounds of the array A, and x has been chosen as the offset from array A to the value of the secret that the attacker should not have access to. As the length of array A has been evicted to main memory by the attacker, Section B will be allowed to execute incorrectly until it returns from memory. Section B then runs the rest of the attack. A byte of the secret is first loaded from the memory, this means that the value of the secret must return from the memory system before the array length. The secret value is then scaled such that each individual value of the secret - 0 to 255 - will each reside on seperate cache lines of the probe array P. In Section C, the attacker will time the accesses of the probe array, and the cache lines corresponding to values that were not the secret must load from main memory and thus take a long time. On the other hand, the value of the secret was transmitted from Section B into the cache state, and the cache line in the probe array that corresponds to the value of the secret will instead load quickly.

\subsection{Example 2: Backward Facing Stateful Inclusive}

\begin{figure}[h]
\begin{verbatim}
       index = B[0]; // traverse linked list
       index2 = B[index]; // index2 == attack
       value = B[index2];
       (mis-speculate) {  // mis-speculated here
           s_bit = bit(*secret, k) // get single bit 
           if(s_bit) { // branch on secret bit
              tmp = B[attack]; // leak secret to cache
           }
       }
\end{verbatim}
\caption{An example of a backwards facing speculative attack.}
\label{fig:spectre_backwards}
\end{figure}

\begin{figure}
    \centering
    \begin{subfigure}[a]{0.5\textwidth}
        \includegraphics[width=\textwidth]{figs/linked_list_zero.png}
        \caption{Secret bit is zero}
        \label{fig:link_list_zero}
    \end{subfigure}
    ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
      %(or a blank line to force the subfigure onto a new line)
      
    \begin{subfigure}[b]{0.5\textwidth}
        \includegraphics[width=\textwidth]{figs/linked_list_one.png}
        \caption{Secret bit is one}
        \label{fig:time_inclusive}
    \end{subfigure}
    \caption{An example of a backwards facing inclusive speculative execution attack. The attack leaks a single bit at a time by modifying the execution time of section A. }
    \label{fig:linked_list}
\end{figure}

The Figure~\ref{fig:spectre_backwards} contains the simplifyed code to execute a backwards facing stateful inclusive attack. This attack attempts to leak a single bit of a secret value, by modifying the execution time of the linked list walk that occurs in Section A. Looking at line 4, we have removed the conditional that contained the bounds check. This has been done, because these attacks are not just limited to Spectre variant 1, but can be applied to any speculative execution attack. Looking at the timing diagram in Figure~\ref{fig:linked_list}, we note that we have also not listed the line of code that causes the mis-speculation. This is to remove clutter from the diagram. It can be assumed that mis-speculation begins when Section B begins, and is resolved when the instructions in section B are squashed. The following sub-sections explain some of the other changes to this diagram.

\subsection{Channel Bit Width}
The speculative execution attack shown in Figure~\ref{fig:spectre_v1} attempts to leak one byte per iteration into the cache state. This can be accomplished because the cache can store at least 2\textsuperscript{8} independent states, which can be measured using 2\textsuperscript{8} independent timing measurements. Multi-bit width side-channels are not required for speculative execution attacks, as we showed in the next example shown in Figure~\ref{fig:linked_list}, here we have leaked a single bit into the cache state. Many side channels can only transfer a single bit at a time, and since that is the most reliable way to transmit over concurrent contention attacks - only using two states, either there is contention or there is no contention - and we can only take a single measurement per attack using inclusive timing strategies, this will be the bit width we use for the remaining of the paper.

\subsection{Checkpointing}
Referring again to Figure~\ref{fig:linked_list}, we see that there is a conditional branch within the mis-speculation. As this conditional branch will also be predicted by the branch predictor, the attacker must train the branch to predict false - by using training values that contain the bit values of 0 - otherwise the branch could mis-speculate as true, and incorrectly modify the execution time of Section A. While the branch is almost always predicted as false, the value of the secret bit should evaluate before the malicious mis-speculation, and the processor can use a technique called checkpointing - saving checkpoints for individual branches and immediately squashing and recovering from mis-speculated branches - to execute the instructions associated with a secret bit value of 1. We witness checkpointing, while performing our attacks, on all tested commodity processors. While not necessary for all concurrent contention attacks, we will adopt this secret bit branching strategy in all further examples. Thus, to save space an lessen diagram complexity, in future diagrams, we omit the bit test, and only show the instructions in Section B that execute under the secret bit value of 1 condition.

\subsection{Concurrent Contention After Squashing}
Again, returning to Figure~\ref{fig:linked_list}, note that we have added a red box with a dotted boundary to Section B. While the bottom of the solid red box represents when the instructions of Section B have become squashed, the bottom of the dashed box represents when their resource requests have finally terminated. Because these resource requests - such as memory accesses - remain in-flight, these already squashed instructions still have potential to cause concurrent contention on the system.

==> oldfiles/Desgin-example.tex <==

\subsection{Example}

\begin{figure*}[htp]
    \centering
    \begin{subfigure}[b]{0.95\textwidth}
        \includegraphics[width=\textwidth]{figs/attack_diagram_0.png}
        \caption{Sending a '0' over the covert channel}
        \label{fig:attack_diagram_0}
    \end{subfigure}
    \begin{subfigure}[b]{0.95\textwidth}
        \includegraphics[width=\textwidth]{figs/attack_diagram_1.png}
        \caption{Sending a '1' over the covert channel}
        \label{fig:attack_diagram_1}
    \end{subfigure}
    \caption{ Diagram \fixme{update the caption}}
    \label{fig:attack_diagram}
\end{figure*}

Figure~\ref{fig:attack_diagram} provides an example using SpectreRewind with a functional unit that is not fully pipelined. 
For our covert channel, we will only send 1 bit at a time, a bit value of `0' will be sent by no contention on the functional unit, and a bit value of `1' will be sent by causing contention on the functional unit. 

The µops0-2 are all using the shared functional unit that consists of 2 non-uniform stages, The first stage takes 3 clock cycles to complete---counting the red "issue" cycle, while the second stage only takes 1 cycle. The µops0-2 are also dependent on one another, causing a long total number of clock cycles to execute. The µop3 causes a branch that is dependent on the results of µops0-2 and has been trained to mis-speculate---note this setup is not a Spectre attack, it is contrived to create transient instructions while remaining simple. 
µops4-5 occur during the transient execution phase of the covert channel. 
Between µop3 and µop4, there are actually important omitted µops---that have been omitted to keep the diagram simple and readable. These µops read single bit of message to transmit and branch based on value of bit. This branch has been initially trained to be not taken---send a '0'. 

Figure~\ref{fig:attack_diagram_0} shows the scenario where that prediction was correct, and 2 µops are executed that use a different functional unit than the one that µops0-2 are using, thus these µops do not contend for the functional unit. Finally, µop6 is a serializing timing instruction that waits for µop3 to complete before executing taking a time measurement.

Figure~\ref{fig:attack_diagram_1} represents the scenario where the prediction was incorrect and a '1' value should be sent over the covert channel. In this scenario, because the prediction of the omitted branch µop is incorrect, the two µops that used the non-competing functional unit from the `0' scenario are squashed---also omitted for diagram simplicity---before fetching 2 µops that use the same functional unit as µops0-2---labeled µop4-5. These µops are now able to contend for the functional unit as depicted by the arrows. Once µop0 is completed in stage 1 of the unit, µop4 is the next ready instruction and is able to enter stage 1. The µop1 then becomes ready but must wait for µop4 to exit stage 1 before it may be issued successfully delaying µop1 for 2 clock cycles---the same scenario that is shown in Figure~\ref{fig:func_try_C}. The same process is then repeated to delay µop2, causing the entire process to take an additional 4 clock cycles which is measurable by the timer, and thus visible to the architecture.

==> oldfiles/Design-older_instr.tex <==
\subsection{Targeting Older Instructions}

\begin{figure}[htp]
  \includegraphics[width=0.5\textwidth]{figs/attack_problems.png}
  \caption{Simplified timing diagram of transient execution attack }
  \label{fig:covert_timing}
\end{figure}

Figure~\ref{fig:covert_timing} is used to demonstrate motivation of our design. This figure shows a timing diagram for an out-of-order processor core similar to that shown in Figure~\ref{fig:backend}. In the diagram, each horizontal line represents an individual µop as it moves through the different stages of the processor core, and each individual box on that line represents a clock cycle tick of the core. This figure also shows a transient execution attack. The µop5 is mis-predicted causing transient execution and µops6-7 are the transient µops that have access to secret---notice that these µops are squashed and not retired to the architectural state. The µops0-2 represent µops that are logically before---in program order---the µop that caused transient execution, while µop9 is logically after. We omit µops 3, 4, and 8 as they are not important to the attack, and to highlight that attack need not be sequential µops. The uops6-7 will be terminated at squash, and thus execution time will not be visible to architecture. The µops 0, 1, 2, 5, and 9 all become architecturally visible, so the attacker's goal will be to modify the execution time of one of these µops based on value of secret. We would like to read from covert channel during transient execution, so particularly we wish to modify execution time of µops before squash happens.

Our design is based on 3 key observations---numbered in the Figure~\ref{fig:covert_timing}. First, µops that occur logically after transient execution(µop9) in program order do not execute before squash. Second, µops that come logically before transient execution (µops0-2) can be executed before squash, and thus transient instructions (µops6-7) have potential to modify their execution times before squash. Third, if the total time taken to execute µops0-2 overshadows the transient execution and following µops(9) are dependent on µops0-2, changes in the timing of these µops(0-2) will be visible in the timing of the entire attack. 
% concurrently with transient execution. Our goal is to modify execution  we can see that µops6-7 will not be able to cause simultaneous contention with µop9---or any µops that logically follow transient execution in program order---this happens because once µop5 executes and realizes the prediction that caused µops6-7 to be fetched was incorrect, the processor will squash these µops and they will no longer be utilizing execution resources by the time logically correct µops---like µop9---are fetched and executed. We also see that µops within the transient execution window cannot extend the window by trying to perform long tasks. This can be seen from µop7 that is attempting to extend the transient execution window by using a functional unit that takes many clock cycles, but it is simply squashed at the same time it would be if it had ran quickly like µop6. This leaves µops0-5 that the transient instructions can attempt concurrent contention with. µop0-2 are dependent on one another---do not issue until the previous one has completed---and thus are taking many clock cycles to execute. This allows their execution to overlap with the execution of the transient instructions (2) and thus they many be able to cause simultaneous contention with them. Finally, we note that (3) if µop0-2 execution takes more cycles than the transient execution attack, and µop9 is either a serializing timing instruction that waits for all other instructions to execute before running or is dependent on µop2, that it will actually time µops 0-2 and detect any timing variations caused by the transient execution attack.
Thus, our framework will attempt to modify the execution times of µops that happen logically before transient execution in program order, in order to create a covert channel.


==> oldfiles/DesignMDS.tex <==
\section{SpectreRewindMDS Design}\label{sec:DesignMDS}

==> oldfiles/FustCovert.tex <==
\section{Fust Covert Channel}\label{sec:FustCovert}

In this section, we will show what are the conditions for using Fust (Functional Unit contention on a Single hardware thread from Transient execution) as a covert channel, and present test code which can detect such a channel. We then explore this channel's properties utilizing floating point division on a variety of systems.

\subsection{Differences With Multi-Threaded Hardware}

Simultaneously multi-threaded systems allow multiple instruction streams to execute on the same physical processor core concurrently. This allows the two threads to share costly resources that may be under-utilized - such as the functional units. Because the resources are shared, covert channels can be created by causing contention on the resources, resulting in measurable variability on shared resource throughput. Fust covert channels operate on a single hardware thread, and thus the sender and receiver must both exist within the same instruction stream. They also require that the sender transmit from a transient execution context - instructions will be squashed - and the receiver must retrieve from an architecturally visible context - instructions that will not be squashed.

\subsection{Fust Channel Example}
The code in Figure~\ref{fig:func_covert_code} shows the code that can be used to test the side channel on systems in an architecture portable fashion. 

\begin{figure}[htp]
  \includegraphics[width=0.5\textwidth]{figs/Execution_Overview.png}
  \caption{Basic diagram of how functional units are organized in an out-of-order CPU. }
  \label{fig:exec_overview}
\end{figure}

\begin{figure}
    \centering
    \begin{subfigure}[a]{0.5\textwidth}
        \includegraphics[width=\textwidth]{figs/func_fail_a.png}
        \caption{}
        \label{fig:func_fail_a}
    \end{subfigure}
    ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
      %(or a blank line to force the subfigure onto a new line)
      
    \begin{subfigure}[b]{0.5\textwidth}
        \includegraphics[width=\textwidth]{figs/func_fail_b.png}
        \caption{}
        \label{fig:func_fail_b}
    \end{subfigure}
    \caption{Malicious micro-operation trying to delay the victim using a floating point divider. Because the victim's micro-operations are older than the attacker, the victim is scheduled first, and the attack fails. }
    \label{fig:func_fail}
\end{figure}

\begin{figure}
    \centering
    \begin{subfigure}[a]{0.5\textwidth}
        \includegraphics[width=\textwidth]{figs/func_win_a.png}
        \caption{}
        \label{fig:func_fail_a}
    \end{subfigure}
    ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
      %(or a blank line to force the subfigure onto a new line)
      
    \begin{subfigure}[b]{0.5\textwidth}
        \includegraphics[width=\textwidth]{figs/func_win_b.png}
        \caption{}
        \label{fig:func_fail_b}
    \end{subfigure}
    ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
      %(or a blank line to force the subfigure onto a new line)
      
    \begin{subfigure}[b]{0.5\textwidth}
        \includegraphics[width=\textwidth]{figs/func_win_c.png}
        \caption{}
        \label{fig:func_fail_c}
    \end{subfigure}
    \caption{Malicious micro-operation trying to delay the victim using a floating point divider. Although the victim's micro-operations are older than the attacker the victim is still waiting on its dependency from the last request, the attacker is scheduled first, and the attack succeeds. }
    \label{fig:func_fail}
\end{figure}

\begin{figure}[htp]
  \includegraphics[width=0.5\textwidth]{figs/func_timing.png}
  \caption{Timing diagram for functional unit concurrent contention attack.}
  \label{fig:func_attack_timing}
\end{figure}

\begin{figure}
    \centering
    \begin{subfigure}[a]{0.5\textwidth}
        \includegraphics[width=\textwidth]{figs/kaby.pdf}
        \caption{Kaby Lake Microarchitecture}
        \label{fig:time_kaby}
    \end{subfigure}
    ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
      %(or a blank line to force the subfigure onto a new line)
      
    \begin{subfigure}[b]{0.5\textwidth}
        \includegraphics[width=\textwidth]{figs/broadwell.pdf}
        \caption{Broadwll Microarchitecture}
        \label{fig:time_broadwell}
    \end{subfigure}
    ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
      %(or a blank line to force the subfigure onto a new line)
      
    \begin{subfigure}[c]{0.5\textwidth}
        \includegraphics[width=\textwidth]{figs/zen.pdf}
        \caption{Zen Microarchitecture}
        \label{fig:time_zen}
    \end{subfigure}
    \caption{ Fust covert channel difference between sending a '0' and a '1' bit on multiple systems taking 300,000 samples. While the channel has low noise on each system, each system has vastly different properties. }
    \label{fig:time_micro}
\end{figure}



==> reviews.tex <==
\appendix
\section{Addressing Review}

To address the following reviews, we began by improving our implemented attacks section. In the first version of the paper, we only implemented the POC native code showing that the covert channel was possible. We have now applied the channel to Meltdown attacks, and implemented the channel in Google Chrome Sandbox.

We doubled the amount of systems that we tested the channel on, including an ARM architecture. Also, writing quality and related works have been improved.

\section{Usenix Security Reviews}

Review \#1229A
==================================

Review recommendation
---------------------
2. Reject and resubmit

Writing quality
---------------
2. Needs improvement

Reviewer interest
-----------------
2. I might go to a talk about this

Reviewer expertise
------------------
4. Expert

Paper summary
-------------
In this paper, the authors describe a contention-based covert channel that can be utilized in transient execution attacks. While contention-based covert channels have been described in recent related work ([4,5]), the described channel is designed to be used on a single hardware thread instead of an SMT setting. The authors evaluate the performance and error rate of their DIVSD covert channel.

Strengths
---------
* Limited same-thread covert channel

Weaknesses
----------
* SpectreRewind is presented as an entire framework despite being just a covert channel
* The covert channel is not very well evaluated
* Covert channel is initiated only with DIVSD instructions
* The attack evaluation is very limited
* More effort should be put into the text, citations, and figures of the paper

Please see the detailed comments for more explanation.

Detailed comments for authors
-----------------------------
The paper describes SpectreRewind as an entire framework, which is a bit misleading as I, as a reader, expect more of it than just being a covert channel that can be utilized in transient execution attacks in a limited way. While some of its limitations are described in the paper, there are some other areas that can be improved throughout the paper.

\#\#\# Attack Scenarios

The paper has an interesting idea to establish a contention-based covert channel by issuing the necessary instructions before the victim code. However, the scenarios in which it can be used as well as its evaluation is rather limited. In Section 6.2, you describe a native code attack where you evaluate a Spectre V1 gadget within the same application. Please give the measured performance numbers and describe in which setting this attack can be realistic because in Section 6.4, you mention that a cross-process or a context-switch attack is not possible. Your reasoning of 'as we require the covert channel to be both written too and read from simultaneously' is not clear. Can't you issue your instructions before using a syscall to jump into the kernel where you have instantly a Spectre V1 gadget (custom kernel module) before returning to your attacking application? How long is the transient window that allows you to use your covert channel?

In Section 6.2, you describe a sandboxed (JavaScript) setting, but you did not evaluate it and mention it in future work. It would be great if you would evaluate your covert channel also in this setting.

\#\#\# Mitigations

While you describe several hardware mitigations and discuss your covert channel with them in-place, I would like to see a discussion with the following publications and patent: Intel describes in 'A New Memory Type against Speculative Side Channel Attacks' [A] the introduction of a new memory type *SAPM* as a solution for multiple transient execution attacks. NVIDIA filed a patent "Memory Type which is cacheable yet inaccessible by speculative instructions" [B] with a similar approach. In addition, the academic publication ConTExT [C] describes an approach that also works on registers. Would these designs mitigate your described attacks?

\#\#\# Other

* "to the provided framework": By reading the paper, describing SpectreRewind as an entire framework seems to be exaggerated as it more or less is just a covert channel (as it is said in the Conclusion). Did you develop an entire framework around this, and is the source of this framework available?
* Please work over the text as some sentences contain grammar mistakes and are hard to read. Please try to avoid the extensive use of "---" for inserted sentences.
* Please work over the figures. Figure 1 and Figure 7 use way too much space.
* Please make sure to cite where appropriate. In 2.1, there is not a single citation. In Section 6.2, you describe the number of uops within the ROB. Where are those numbers from? In the introduction, you mention "most defense mechanisms", please already give citations here.
* In 2.2, you describe that the data leaked with MDS attacks comes from other SMT threads. The data can also come from the same hardware thread that previously executed in a privileged context, so SMT is not a necessity for those attacks.
* In the threat model, you state: "We assume that the attacker cannot successfully either create or coordinate with other attacker controlled threads or processes that are running on the same system" - Why is that the case?
* You also state that "the attacker would like to construct code that will transmit the secret over a covert channel" - This is your described covert channel?
* In 4.1, you describe non-pipelined functional units. In Section 5, you decide to use the floating-point division unit. How did you evaluate that it is not fully pipelined? Is this documented somewhere? What other units could I use for such a covert channel? Which other instructions could I use, and how do they compare to each other? This could yield some interesting additional results.
* In Section 5.2, you describe that you recalibrate the thresholds for every bit you transmit. Why is this necessary? Could you not calibrate your covert channel once?
* In Section 5.2, you require the transmitter to repeat sending the same bit multiple times. The reason is that RDTSC increments only every ~20-30 cycles depending on the AMD microarchitecture since Zen. Other publications fall back to a counting thread in this scenario. Can you achieve a higher transmission rate with such a timing primitive?

\#\#\# Nitpicks:

* P2: "of a Spectre based transient" -> "Spectre-based"
* P2: "ReOrder Buffer(ROB)" -> Missing space
* P3: "are differed" -> "are deferred"
* P3: "technically meltdown type" -> "Meltdown-type"
* P4: "with other attacker controlled threads" -> "attacker-controlled"
* P5: "In Figure 5a, We" -> "we"
* P6: "secret dependent timing" -> "secret-dependent"

\#\#\#\# References

* [A] https://nam10.safelinks.protection.outlook.com/?url=https%3A%2F%2Fgithub.com%2Fintelstormteam%2FPapers%2Fblob%2Fmaster%2F2019-A_New_Memory_Type_Against_Speculative_Side_Channel_Attacks.pdf&amp;data=02%7C01%7Cjacobfustos%40ku.edu%7Cdd92134f3ba948672f4908d7cd54ad78%7C3c176536afe643f5b96636feabbe3c1a%7C0%7C1%7C637203635891393135&amp;sdata=ZQ88PihyfhscxOmpfJOPWzyZFABavyc6j61uEcVfzF0%3D&amp;reserved=0
* [B] https://nam10.safelinks.protection.outlook.com/?url=https%3A%2F%2Fpatentscope.wipo.int%2Fsearch%2Fen%2Fdetail.jsf%3FdocId%3DUS235550717&amp;data=02%7C01%7Cjacobfustos%40ku.edu%7Cdd92134f3ba948672f4908d7cd54ad78%7C3c176536afe643f5b96636feabbe3c1a%7C0%7C1%7C637203635891393135&amp;sdata=LU11sZguQFM5Ws65DVujo3yLtujwp6FLEt5Qes56gsM%3D&amp;reserved=0
* [C] https://nam10.safelinks.protection.outlook.com/?url=https%3A%2F%2Fwww.ndss-symposium.org%2Fndss-paper%2Fcontext-a-generic-approach-for-mitigating-spectre%2F&amp;data=02%7C01%7Cjacobfustos%40ku.edu%7Cdd92134f3ba948672f4908d7cd54ad78%7C3c176536afe643f5b96636feabbe3c1a%7C0%7C1%7C637203635891393135&amp;sdata=u6qR0Ij%2F2P2XHFSx6%2FyE%2F8SRZtRuZTreC23cVev0ifU%3D&amp;reserved=0


* * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * *


Review \#1229B
===========================

Review recommendation
---------------------
2. Reject and resubmit

Writing quality
---------------
3. Adequate

Reviewer interest
-----------------
3. I would definitely go to this talk and tell my students or colleagues to
   read this paper

Reviewer expertise
------------------
3. Knowledgeable

Paper summary
-------------
The paper presents SpectreRewind, a new covert channel for transient execution attacks that exploits contention with transiently executed subsequent instructions. The authors instantiate the channel using floating-point division instructions, and measure its performance, showing transfer rates of over 1000 bits/second with a negligible error rate

Strengths
---------
* Nice new channel

Weaknesses
----------
* No actual attack - the security threat is not clear

Detailed comments for authors
-----------------------------
I enjoyed reading the paper.  the covert channel is really nice, and I would really like to see this published.  Unfortunately, the work feels incomplete.  As written it can be a very nice workshop paper, but does not reach the bar for USENIX Security.

The main limitation of the work is that the security threat it poses is not clear. There are two scenarios where the attack has a potential - for implementing Meltdown-type attacks in the presence of shadow buffers, and for implementing Spectre attacks in sandboxes. However, the paper evaluates the attack in neither scenarios.  The former is a bit difficult, because the defenses do not yet exist. The latter, however, is promising.  I recommend that the authors demonstrate an attack on JavaScript.  I also note that SpectreRewind can bypass some defenses that strategically add fence instructions inside what looks like Spectre gadgets.  Thus, it may be possible to show an attack that bypasses current defenses.  Based on the information in the paper, it is not clear how much work would be required for a JavaScript attack, or if such an attack is at all feasible.  As such, I am reluctant to recommend a major revision.

The demonstration of the attack only uses floating point divisions. Are there other instructions that can be used for the attack?  Any method of identifying such instructions?

It may be worth noting that the CacheOut attack (https://nam10.safelinks.protection.outlook.com/?url=https%3A%2F%2Fcacheoutattck.com&amp;data=02%7C01%7Cjacobfustos%40ku.edu%7Cdd92134f3ba948672f4908d7cd54ad78%7C3c176536afe643f5b96636feabbe3c1a%7C0%7C1%7C637203635891393135&amp;sdata=j8acNhelq9iRa9ZmtkH%2B1ct40IC3UeejZU%2BOhWyP5Nc%3D&amp;reserved=0) also exploits reversal of execution order, albeit for a different purpose than SpectreRewind.

***Minor Comments***
- Page 1: ... as a viable covert channel --> is a viable
- Page 2: effecting their execution time --> affecting
- Page 2: once its operands --> their
- Page 3: You may want to add line numbers in Figure 2 to facilitate referencing
- Page 3: (Nit picking) Contrary to what the paper claims, the state of the cache is not visible to architecturally visible instructions. The attacker recovers it through first translating it to timing or to performance counters information, which is architecturally visible.
- Page 3: I am not sure why the paper distinguish MDS attacks from other Meltdown-type attacks.
- Page 5: shared functional unit that is non-pipelined(stage 1... -->  non-pipelined shared functional unit (stage 1...
- Line 9 of Figure 6: prove --> probe
- Page 6: before it can entering --> before entering
- Page 6: '0', '1' --> `0', `1' --- in multiple places
- Table 1: 13-15 --> 13--15.  Same for other columns
- Figure 7: When printed in B/W I cannot distinguish the green and purple lines
- Section 5.2 overloads the term 'throughput'.  I suggest using 'transfer rate' when referring to the covert channel capacity, as in Table 1.
- The caption of Figure 8 is not a full sentence.
- Page 8: form security scanning algorithms --> from
- Page 8: written too and read from --> to
- KB and MB typically refer to Kilobyte and Megabyte.
- [4,6,17]: Please cite the peer-reviewed conference publications rather than the preprints

Requested changes
-----------------
* Implement a sandboxed attack
* Investigate the use of other instructions for the attack

Questions for authors' response
-------------------------------
Have you tried a sandboxed attack?  Any results so far?
